A Universal Technique for Machine-Certified Proofs of Linearizable Algorithms

Linearizability has been the long standing gold standard for consistency in concurrent data structures. However, proofs of linearizability can be long and intricate, hard to produce, and extremely time consuming even to verify. In this work, we address this issue by introducing simple $universal$, $sound$, and $complete$ proof methods for producing machine-verifiable proofs of linearizability and its close cousin, strong linearizability. Universality means that our method works for any object type; soundness means that an algorithm can be proved correct by our method only if it is linearizable (resp. strong linearizable); and completeness means that any linearizable (resp. strong linearizable) implementation can be proved so using our method. We demonstrate the simplicity and power of our method by producing proofs of linearizability for the Herlihy-Wing queue and Jayanti's single-scanner snapshot, as well as a proof of strong linearizability of the Jayanti-Tarjan union-find object. All three of these proofs are machine-verified by TLAPS (the Temporal Logic of Actions Proof System).

==> examples/queue-old.tex <==
\section{Example: Queue}

In this section, we consider Herlihy and Wing's implementation of a queue object \cite{HW90} and describe our machine-verified proof of its linearizability with the use of TLAPS \cite{TLAPS}.
As part of their seminal work renowned for defining the concept of linearizability, Herlihy and Wing also provide a linearizable queue implementation. The proof the implementation's linearizability is significantly more elaborate than the implementation itself, and hence appeared to us as an ideal candidate for the application of our technique.
% Why did we choose this algorithm?

\subsection{The Queue Type}
The queue type maintains elements from $\mathbb{N}^+$ in a sequence and supports two operations.
\begin{itemize}
    \item 
    $\Enqueue(v)$ adds $v$ to the end of the sequence.
    \item
    $\Dequeue()$ removes and returns the first element in the sequence, when the sequence is not empty.
    % How should I handle the case when the queue is empty?
\end{itemize}
We already provided the full formal specification of the queue type in the figure Object Type~\ref{type:queue}.
% \subimport{object-types}{queue}

\subsection{The Herlihy-Wing Queue Implementation}

We present Herlihy and Wing's queue implementation in Figure~\ref{impl:queue}.
As before, each numbered line acts on at most one shared memory instruction, and is performed atomically.

\subimport{implementations}{queue}

We shall now briefly explain the algorithm. $X$ denotes the foremost unused index of $Q$. An enqueuing process $\pi$ stores $X$ in $i_{\pi}$, and increments $X$. $i_{\pi}$ is the index of $Q$ that $\pi$ has claimed for use, specifically for the storage of its argument $v_{\pi}$. $\pi$ then simply writes $v_{\pi}$ in $Q[i_{\pi}]$ and returns. A dequeuing process $\pi$ starts by reading $X$ into $l_{\pi}$; at which point indices $1$ through $l_{\pi} - 1$ are determined to be the indices of $Q$ that $\pi$ will look through to find the first non-$\bot$ value to dequeue. If $l_{\pi} = 1$, there are no indices to consider, and therefore the procedure is restarted and the program counter is reverted to line $6$. $\pi$ iterates through the determined set of indices (using the loop variable $j_{\pi}$) and reads each value $Q[j_{\pi}]$ into $x_{\pi}$. If any non-$\bot$ value is detected, $x_{\pi}$ is returned; otherwise, if $j_{\pi} = l_{\pi} - 1$, as this indicates that we have exhausted all considered indices without finding a stored value, the procedure is restarted.

\subsection{The Tracker}
A partial tracker for the Herlihy-Wing queue implementation is provided in Figure~\ref{impl:queue-tracker}, which, by Theorem~\ref{thm:partial-tracker}, suffices to prove the linearizability of the implementation if it has $\M \neq \emptyset$ as an invariant.
The tracker we propose is as follows: 
\begin{itemize}
    \item For a process $\pi$ at line 2, for each meta-configuration in $\M$, we allow the linearization of any subset of unlinearized $\Enqueue$ operations that are past line 2 (or $\pi$'s own operation) in any order, to create new meta-configurations.
    \item For a process $\pi$ at line 8, if $x_{\pi}$ is not $\bot$ (after the read), we simply linearize $\pi$'s $\Dequeue$ operation to create new meta-configurations.
    \item At both invocation lines, we consider the meta-configurations that result from the invocation taking place (linearizing an empty sequence of processes). At both return lines, we choose all meta-configurations that result from the return. For every remaining intermediate line, we simply linearize the empty sequence of processes.
\end{itemize}

\subimport{implementations}{queue-tracker}

\subsection{Proving The Invariant}
We seek to prove that $\I_{L} \equiv \M \ne \nullset$ is an invariant.
$\I_L$ clearly holds in the initial configuration of the algorithm, so it suffices to show that it will continue to hold in subsequent configurations; we will accomplish this task by induction.
Of course, $\I_L$'s validity in subsequent configurations of the algorithm relies not only on its validity in the current state, but also on the design of the algorithm, i.e. other invariants of the algorithm that capture the states of the various program variables (objects and registers).

Thus, in order to go through with our strategy, we must strengthen $\I_L$ to a stronger invariant $\I$ that meets two conditions: 
(1) $\I$ is {\em inductive} and (2) $\I$ implies $\I_L$.
This task of strengthening $\I_L$ to an $\I$ that meets the conditions is the main intellectual work that the prover must do.
In particular, the identification of $\I$ requires an understanding of ``why the algorithm works'', and thus the {\em prover} ({\em unlike the verifier}) must still, in general, understand the algorithm well in order to give the proof.

In the case of the Herlihy-Wing queue implementation, we present the strengthened invariant $\I$ in Figure~\ref{inv:queue}. $\I$ is a conjunction, with $\I_L$ among its conjuncts.
Thus, when we prove its invariance, we have $\I_L$ by implication.
The remaining conjuncts can be understood as follows:
\begin{itemize}
    \item The conjuncts $\I_X, \I_Q, \I_v, \I_i, \I_l, \I_j, \I_x, \I_{pc}, \I_{\M}$ express type safety. 
    That is, the various variables in the algorithm always take on values that we would expect satisfy their types. 
    \item The conjuncts $\I_{1, 5}, \I_2, \I_3, \I_4, \I_6, \I_7, \I_8, \I_9$ express truths that pertain to a process $\pi$ when its program counter $pc_{\pi}$ has a particular value, both regarding the meta-configurations permitted by the suggested tracker, as well as the values of the variables of the original implementation.
    \item The conjuncts $\I_a$ and $\I_b$ express general truths about the implementation and the tracker. $\I_a$ asserts that for any index $k$ of $Q$ greater than $X - 1$, it is the case that $Q[k] = \bot$, which should be trivial since $X$ denotes the foremost unused index of $Q$. The discussion of $\I_b$ requires defining a number of additional predicates first.
\end{itemize}
\subimport{invariants}{queue-tracker}

Let us first define a predicate $GoodEnqSet$ that, given a set $A$ of indices between $1$ and $X-1$, 
determines whether the set can correspond to a set of linearized $\Enqueue$ operations.
If an index $k \in [X-1]$ corresponds to a non-$\bot$ element stored in $Q$, then it is linearized and must appear in $A$.
Otherwise, an index $k$ that appears in $A$ and is such that $Q[k] = \bot$, must appear in $A$ by virtue of the existence of a process $\pi$ at line 3, that has claimed $k$ as the index of $Q$ it will write its argument into.
We can then formally define $GoodEnqSet(A)$ for any $A \subseteq [X-1]$ as follows:
\begin{align*}
GoodEnqSet(A) \triangleq \forall k \in [X-1] : \ & (Q[k] \neq \bot \implies k \in A) \\ &\wedge ((Q[k] = \bot \wedge k \in A) \implies \exists \pi' \in \Pi : pc_{\pi'} = 3 \wedge i_{\pi'} = k).
\end{align*}

Let us then consider the responses processes should receive under specific linearizations. If a process $\pi$ is at line 4 or 9, its operation must have been linearized and the process must have been assigned a return value of either $\ack$ or $x_{\pi}$, respectively for $\Enqueue$ and $\Dequeue$. Moreover, it must have been assigned a response value of $\ack$ at line 3 if $\pi$, or some other process, linearized $\pi$'s $\Enqueue$ as part of their update to $\M$ in line 2. With this observation, let $A$ be a conjectured set of the indices of $Q$ between $1$ and $X-1$, claimed for use by the linearized $\Enqueue$ operations.
Then, any $\pi$ at line 3 whose picked index $i_{\pi}$ appears in $A$, must also be linearized and also assigned a return value of $\ack$. Besides these three cases, no other processes are assigned return values.
In the light of these observations, for a conjectured set of linearized $\Enqueue$ indices $A \subseteq [X-1]$ and a meta-configuration $C \in \M$, let us define the predicate $GoodRes(A, C)$ which indicates that the response field of $C.f$ has return values that correspond to the linearizations conjectured by $A$:
\begin{align*}
    GoodRes(A, C) \triangleq \forall \pi' \in \Pi: C.f.ret = \begin{cases}
        \ack     & \text{if } pc_{\pi'} = 3 \wedge i_{\pi'} \in A \\
        \ack     & \text{if } pc_{\pi'} = 4 \\
        x_{\pi'} & \text{if } pc_{\pi'} = 9 \\
        \bot     & \text{otherwise.}
    \end{cases}
\end{align*}

Akin to how we define a valid correspondence between the response field of meta-configurations in $\M$ and return values resulting from particular conjectured linearizations in $GoodRes$, we can also define a correspondence between the state fields of meta-configurations and the values of variables in the implementation.
If for a permutation $s$ of a set $A \subset [X-1]$ of the conjectured set of indices claimed for use by the linearized $\Enqueue$ operations, then the state of the implemented object should be a sequence of values pointed to by the indices (or in the case where the value pointed to by the index is $\bot$, the argument of the process having picked the given index), in the order the indices appear in $s$. Then, for any $s \in Perm(A)$ where $A \subseteq [X-1]$ and a meta-configuration $C \in \M$, let us define the predicate $ValuesMatchInds(s, C)$, which indicates that $C.\sigma$ indeed corresponds to the order of linearizations conjectured by the sequence of indices $s$:
\begin{align*}
    ValuesMatchInds(s, C) \triangleq
    C.\sigma = \left(
    k \in [|s|] \mapsto
    \begin{cases}
        Q[s_k] & \text{if } Q[s_k] \neq \bot \\
        v_{\pi'} & \text{where } \pi' \in \Pi : pc_{\pi'} = 3 \wedge i_{\pi'} = s_{k}
    \end{cases}
    \right).
\end{align*}
We note that this is a well-defined expression for all $A$ where $GoodEnqSet(A)$ holds true, as this would (along with invariant $\I_3$) guarantee the existence of a unique process $\pi'$ where the second case is applicable.

For the final necessary definition, let us once again consider a permutation $s$ of a set $A \subset [X-1]$ of the conjectured set of indices claimed for use by the linearized $\Enqueue$ operations, and reflect about what might render $s$ a potentially correct sequence of linearizations.
Before all else, if $s$ simply is the non-empty indices of $Q$ in the order in which they appear in $Q$, it should clearly be represent a potentially correct sequence of linearizations, since an incoming dequeuing process can execute successive $\Dequeue$ operations and indeed empty the queue in this order, meaning that this sequence corresponds to a potentially correct state of the implemented object.
Let us consider the cases where $s$ does not follow this order, and suppose it contains a pair of indices $m, n$ such that $n < m$ yet $s_m < s_n$.
In this case, if $s_m$ points to an empty component in $Q$,
$s$ constitutes a potentially correct ordering of the indices, as a dequeuing process might very well pass through $s_m$ as it loops through indices, before reaching $s_n$.
However, if $Q[s_m] \neq \bot$, it is not immediately clear whether $s$ is a potentially correct ordering.
In order to be able to assert this, we must ensure that there is a dequeuing process $\pi$ which is past $s_m$ in its loop (i.e. $s_m < j_{\pi}$), such that $s_n < l_{\pi}$ (which would otherwise fall outside the scope of indices $\pi$ could dequeue from).

Then, to capture this idea, let an \textit{inversion} for a sequence $s$ of indices of $Q$, denote a pair $m, n \in |s|$ for which $n < m, s_m < s_n$ and $Q[s_m] \neq \bot$.
For a sequence of indices to correspond to a potentially correct sequence of linearizations, the inversions it contains must all be \textit{justified}. A \textit{justified inversion}, as discussed in the preceding paragraph, is an inversion for which there is a dequeueing process $\pi$ at line 8, for which $s_n < l_{\pi}$ and $s_m < j_{\pi}$.
We can formally define this as a predicate $JInvSeq(s)$, for $s \in Perm(A)$ for some $A \subseteq [X-1]$, as follows:
\begin{align*}
    JInvSeq(s) \triangleq
    \forall m, n \in [|s|] : (n < m &\wedge s_m < s_n \wedge Q[s_m] \neq \bot) \\ &\implies (\exists \pi' \in \Pi : pc_{\pi'} = 8 \wedge s_n < l_{\pi'} \wedge s_m < j_{\pi'}).
\end{align*}

This completes the definition of $\I$. Our intricate proof that $\I$ is indeed an inductive invariant of the system and proofs of the straightforward deductions that $\I$'s invariance implies the invariance of $\I_L$, thereby proving the strong linearizability of the union find implementation can be found at: 

{\scriptsize
\url{https://github.com/uguryavuz/easy-to-verify-linearizability/blob/main/HWQueue2.tla}
}


% \begin{itemize}
    % \item 
    % Let us first define a predicate $GoodEnqSet$ that, given a set $A$ of indices between $1$ and $X-1$, 
    % determines whether the set can correspond to a set of linearized $\Enqueue$ operations.
    % If an index $k \in [X-1]$ corresponds to a non-$\bot$ element stored in $Q$, then it is linearized and must appear in $A$.
    % Otherwise, an index $k$ that appears in $A$ and is such that $Q[k] = \bot$, must appear in $A$ by virtue of the existence of a process $\pi$ at line 3, that has claimed $k$ as the index of $Q$ it will write its argument into.
    % We can then formally define $GoodEnqSet(A)$ for any $A \subseteq [X-1]$ as follows:
    % \begin{align*}
    % GoodEnqSet(A) \triangleq \forall k \in [X-1] : & (Q[k] \neq \bot \implies k \in A) \\ &\wedge ((Q[k] = \bot \wedge k \in A) \implies \exists \pi' \in \Pi : pc_{\pi'} = 3 \wedge i_{\pi'} = k).
    % \end{align*}
    
    % \item 
    % For $A \subseteq [X-1]$ and $C \in \M$:
    % \begin{align*}
    % GoodRes(A, C) \triangleq \forall \pi' \in \Pi: C.f.ret = \begin{cases}
    %     \ack     & \text{if } pc_{\pi'} = 3 \wedge i_{\pi'} \in A \\
    %     \ack     & \text{if } pc_{\pi'} = 4 \\
    %     x_{\pi'} & \text{if } pc_{\pi'} = 9 \\
    %     \bot     & \text{otherwise}
    % \end{cases}
    % \end{align*}

    % \item
    % For $C \in \M$, and for any $s \in Perm(A)$ for some $A \subseteq [X-1]$:
    % \begin{align*}
    % ValuesMatchInds(s, C) \triangleq
    % C.\sigma = \left(
    % k \in [|s|] \mapsto
    % \begin{cases}
    %     Q[s_k] & \text{if } Q[s_k] \neq \bot \\
    %     v_{\pi'} & \text{where } \pi' \in \Pi : pc_{\pi'} = 3 \wedge i_{\pi'} = s_{k}
    % \end{cases}
    % \right).
    % \end{align*}

    % \item 
    % For any $s \in Perm(A)$ for some $A \subseteq [X-1]$:
    % \begin{align*}
    % JInvSeq(s) \triangleq
    % \forall m, n \in [|s|] : (n < m &\wedge s_m < s_n \wedge Q[s_m] \neq \bot) \\ &\implies (\exists \pi' \in \Pi : pc_{\pi'} = 8 \wedge s_n < l_{\pi'} \wedge s_m < j_{\pi'}).
    % \end{align*}
% \end{itemize}

==> examples/union-find-old.tex <==
\section{Example: The Union Find Object}
\label{sec:union-find}

In this section, we consider Jayanti and Tarjan's concurrent union-find implementation \cite{JT16, JT21}, and describe how we wrote the machine verified proof that it is linearizable, in fact strongly linearizable, using TLAPS (the Temporal Logic of Actions Proof System) \cite{TLAPS}.
We chose Jayanti and Tarjan's algorithm since it is simple (both to understand and in length of code) and highly practical---it is the fastest algorithm for computing connected components of a graph on CPUs \cite{dhulipala2020connectit} and GPUs \cite{GpuUnionFind}, and has several other applications \cite{alistarh2019search}.

\subsection{The Union Find Type}

The union find type maintains a partition of the {\em elements} in $[n] = \{1,2,\ldots,n\}$ and supports two operations.
\begin{itemize}
    \item 
    $\Find(x)$ returns the maximum element in element $x$'s part of the partition.
    \item 
    $\Unite(x,y)$ merges the parts containing $x$ and $y$ if they are different and returns $\ack$.
\end{itemize}
Formally, we specify the partition as a function $\sigma:[n] \to \mathcal{P}([n])$ from the set of elements to the powerset of the set of elements, such that $\sigma(x)$ is the part containing element $x$.
Of course, if two elements $x$ and $y$ are in the same part of the partition, then $\sigma(x) = \sigma(y)$.
We give the full formal specification of the union-find type in the figure Object Type~\ref{type:union-find}.

\import{object-types}{union-find}

\subsection{The Jayanti Tarjan Union Find Implementation}

We present Jayanti and Tarjan's implementation of union-find in Figure~\ref{impl:union-find}.
Each numbered line in the implementation requires the performance of at most one shared memory instruction, and is performed atomically.

\import{implementations}{union-find}

There are two goals to this section:
(1) {\em to convince} the reader (our current verifier) that the implementation in Figure~\ref{impl:union-find} is strongly linearizable;
(2) to {\em describe the process} by which we prove this strong linearizability.
Meeting goal (1) is very simple:
the reader simply needs to verify that Figure~\ref{impl:union-find-tracker} is indeed a partial tracker of this implementation with meta-configuration variable $\M$,
and then to go to:

{\scriptsize \url{https://github.com/visveswara/machine-certified-linearizability/blob/master/UnionFindTracker.tla}} 

\noindent
where we give a machine verified proof that $|\M| = 1$ is an invariant of the partial tracker.
Done!
In particular, the reader {\em does not} need to read or understand the proof of the invariant; in fact, the reader {\em does not} even need to understand the code of the implementation!
It simply suffices to check that the machine has verified the invariant.
Thus, the rest of this section is primarily aimed at meeting goal (2), that is, describing the process by which we---the designers of the proof---went about constructing the partial tracker and what work is involved in producing a proof of the invariant $|\M| = 1$ that the TLAPS proof assistant is able to machine-verify.
We start by describing the union-find implementation.
% Normally, such a proof would require the reader to understand the code of the implementation and an intricate argument about how the code follows certain principles that make it linearizable.
% Using our method however, the reader will not need to understand or examine the code in order to accept its strong linearizability!
% Nevertheless, we provide a description of the implementation below for the interested reader.

In the implementation, each element is represented by a node, and each node $x$ has a parent pointer field $x.par$ that points to another node.
Each part of the partition is represented as a single parent pointer tree, so $\sigma(x) = \sigma(x.par)$, and 
we maintain the invariant that the parent of $x$ is always greater than or equal to $x$ (i.e. $x.par \ge x$).
Thus, the roots of the trees are the largest elements in their respective partition; if $u$ is a root of its tree than $u.par = u$.
In the initial state $\sigma_0$, all elements are in their own singleton part of the partition, i.e. $\forall x \in [n], \sigma_0(x) = \{x\}$.
Correspondingly, the implementation starts with $\forall x \in [n], x.par = x$.

With this representation, a process $\pi$ performs $\Find_\pi(x_\pi)$ by starting a node $u_\pi$ at $x_\pi$ (line 1), walking $u_\pi$ up the parent pointers until it reaches a root (line 2), and returning that root, which must be the maximum element in the set (line 3).

A process $\pi$ performs $\Unite_\pi(x_\pi, y_\pi)$ by starting a node $u_\pi$ at $x_\pi$ and another node $v_\pi$ at $y_\pi$ (line 4).
The implementation ambitiously hopes that the current nodes $u_\pi$ and $v_\pi$ are roots. If so, and if $u_\pi = v_\pi$ then unite has no work to do and proceeds to return (first part of line 5); otherwise, if $u_\pi < v_\pi$, then unite tries to merge the two separate trees by linking $u_\pi$ under $v_\pi$ via a CAS (second part of line 5); in the remaining case that $u_\pi > v_\pi$ it tries to make the link in the other direction (third part of line 5).
If a link gets made, then there is no more work to do so $\pi$ proceeds to return.
Otherwise, the links may have failed since $u_\pi$ or $v_\pi$ was not a root.
In this case, the implementation walks $u_\pi$ up the tree until it is a root (line 6), and does the same for $v_\pi$ (line 7) and tries again (while true loop).
Once one of the three cases on line 5 eventually occurs, $\pi$ returns $\ack$ (line 8).

\subsection{The Tracker}

Having been given the implementation in Figure~\ref{impl:union-find}, we can blindly write down the full tracker for the implementation, and could prove its linearizability by showing the invariance of $\Mfull \ne \nullset$ by appealing to Theorem~\ref{maintheorem}.
However, we will instead go the route of constructing a partial tracker for two reasons:
(1) we would like to prove {\em strong linearizability}, rather than just linearizability, and 
(2) the full tracker exhaustively maintains the set of all possible linearizations of every run by maintaining atomic configurations that arise by every possible set of processes linearizing in every order after every step of the run.
We however, will demonstrate a more insightful understanding of exactly when and how the implemented object linearizes operations.
By embedding this understanding into the partial tracker, we will make our job of proving the invariant easier.

Our key insight into the implementation is our ability to identify a unique linearization point for each operation, as described in the following observation:
% From the description of the code, we posit a unique linearization point for each \Find and \Unite as follows. 
\begin{observation}
\label{obs:linearization-union-find}
For a \Find{}, the last iteration of the loop at line 2 is when $\pi$ discovers that $u_\pi$ is its own parent and thereby the root and maximum value node in its tree; we posit this to be the linearization point of the operation.
For a \Unite{}, the last execution of line 5 is when $\pi$ either discovers that $u_\pi$ and $v_\pi$ are already in the same tree or when $\pi$ successfully links their trees together with a CAS; so we posit this to be the linearization point.
\end{observation}

For now, the linearization points in Observation~\ref{obs:linearization-union-find} are simply an expression of our intuition from an informal understanding of the algorithm.
However, we will use this intuition to design our partial tracker presented in Figure~\ref{impl:union-find-tracker}, and the proof of our tracker's invariants, which we will discuss later, will formalize this understanding.
% We use this intuition/informal understanding of the algorithm's linearization points to design our partial tracker, which is presented as Figure~\ref{impl:union-find-tracker}.

We ensure that our implementation in Figure~\ref{impl:union-find-tracker} meets the definition of a tracker, by ensuring that the meta-configuration variable $\M$ meets the initialization, invocation, intermediate line, and return line criteria.
In particular:

\import{implementations}{union-find-tracker}

\begin{itemize}
    \item[0.]
    Our meta-configuration is initialized to $\M = \{(\sigma_0, f_0)\}$, where $\sigma_0$ is the initial state of the union-find object, and $f_0$ describes each process as initially idle.
    
    \item[1.]
    In each invocation line by a process $\pi$, by the definition of a partial tracker, we can update $\M$ to contain any configurations $C'$ that result from the invocation and an arbitrary sequence of processes that have pending operations linearizing after any $C \in \M$.
    Observation~\ref{obs:linearization-union-find} suggests that we need not think of any operations as linearizing at this line, thus we update $\M$ to contain exactly the subset of configurations which result from the invocation occurring (and the empty sequence of processes linearizing) after some $C \in \M$.
    This can be confirmed by inspecting the augmentations at line 1 (for \Find) and line 4 (for \Unite).

    \item[2.]
    In each intermediate line by a process $\pi$, by the definition of a partial tracker, we can update $\M$ to contain any configurations $C'$ that result from an arbitrary sequence of processes that have pending operations linearizing after any $C \in \M$.
    Observation~\ref{obs:linearization-union-find} suggests that we can consider at most one process linearizing after each line of code.
    In particular, the observation suggests that for \Find, we need to only $\pi$ linearizing at line~2 if $u_\pi = u_\pi.par$ at the time of that line's execution.
    Similarly, for \Unite, we need to only consider $\pi$ linearizing at line~5, and that too only if either $u_\pi = v_\pi$ or if the conditions are such that one of the two CAS operations will succeed on that line.
    We correspondingly design $\M$ to be updated according to these rules at these particular lines.
    Otherwise, we update $\M$ to contain exactly the set of configurations which result from the empty sequence of processes linearizing, i.e., we leave $\M$ unchanged.
    Thus, a simple inspection of the augmentations to lines 2,5,6, and 7 reveals that our augmentation satisfies the intermediate line condition for a tracker.
    
    \item[3.]
    Finally, in each return line, the definition of a tracker allows us to update $\M$ to contain any configurations $C'$ that result from the return and an arbitrary sequence of processes with pending operations linearizing after any configuration $C \in \M$.
    Once again, we respect Observation~\ref{obs:linearization-union-find}, and choose all configurations $C'$ that result from the return (and the empty sequence of processes linearizing thereafter) after each $C \in \M$.
    This is easily confirmed by inspecting the augmentations to lines 3 and 8.
\end{itemize}

By simple inspections, we have verified that the augmentation in Figure~\ref{impl:union-find-tracker} is indeed a tracker of the union find implementation in Figure~\ref{impl:union-find}.
Notably, we did not need to look at or understand the code of the original implementation (beyond mechanically verifying that it was copied-and-pasted to the augmentation properly).
Even so, by Theorem~\ref{thmstronglinearizability}, seeing a certification of the invariant $|\M| = 1$ from a mechanical proof verifier, suffices as a reliable and rigorous proof that the union-find implementation is Strongly Linearizable (and thereby also Linearizable)!

In the remainder of the section, we will describe {\em how} we went about proving that invariant.

\subsection{Proving The Invariant}

% Until now, we have seen that the {\em verification} of linearizability is quite simple, and simply requires a mechanical check that the presented tracker indeed complies with the rules according to Definition~\ref{def:tracker}, and verifying that the machine has indeed verified the proof of $|\M| = 1$ being an invariant.

Our task is to prove that $\I_L \equiv \M \ne \nullset$ and $\I_S \equiv |\M| = 1$ are invariants of $\A(\Oaug)$ in order to deduce that $\O$ is linearizable and strongly linearizable.
Obviously, $\I_S$ implies $\I_L$, so in this example we will focus on $\I_S$, i.e. strong linearizability, alone.

$\I_S$ clearly holds in the initial configuration of the algorithm, so it suffices to show that it will continue to hold in subsequent configurations; we will accomplish this task by induction.
Of course, $\I_S$'s validity in subsequent configurations of the algorithm relies not only on its validity in the current state, but also on the design of the algorithm, i.e. other invariants of the algorithm that capture the states of the various program variables (objects and registers).
Thus, in order to go through with our strategy, we must strengthen $\I_S$ to a stronger invariant $\I$ that meets two conditions: 
(1) $\I$ is {\em inductive} and (2) $\I$ implies $\I_S$.
This task of strengthening $\I_S$ to an $\I$ that meets the conditions is the main intellectual work that the prover must do.
Of course, the prover must subsequently {\em prove} that $\I$ is inductive and implies $\I_S$; but our experience through proving several algorithms suggests that this latter step, while potentially time-taking due to the length of the proof, is generally intellectually easier once the correct $\I$ is identified.
In particular, the identification of $\I$ requires an understanding of ``why the algorithm works'', and thus the {\em prover} ({\em unlike the verifier}) must still, in general, understand the algorithm well in order to give the proof.

In the case of our union find implementation, we present the strengthened invariant $\I$ in Figure~\ref{inv:union-find}.
$\I$ is a conjunction, and two of the conjuncts are $\I_S$ and $\I_L$.
Thus, when we prove it is an invariant, we clearly have $\I_S$ and $\I_L$ by implication.
The remaining conjuncts can be understood as follows:
\begin{itemize}
    \item 
    The conjuncts $\I_{par}, \I_x, \I_y, \I_u, \I_v, \I_{pc}, \I_\M$ express type safety.
    That is, the various variables in the algorithm always take on values that we would expect satisfy their types.
    For instance, $\I_{par}$ expresses that for each node $z \in [n]$, $z.par$ is also a node.
    \item 
    The conjuncts $\I_a, \I_b, \I_c$ express general truths about our union find implementation.
    Namely, that every node $z$ shares a part in the partition with its parent $z.par$;
    that if $z$ and $w$ are different roots, then they are different parts of the partition;
    and that parent pointers never point to smaller valued nodes.
    \item
    The conjuncts $\I_{1,4}, \I_2, \I_3, \I_{5,6,7}, \I_8$ express truths that pertain to a process $\pi$ when its program counter $pc_\pi$ has a particular value.
    For instance, $\I_{5,6,7}$ expresses that if $pc_\pi \in \{5,6,7\}$, then the pairs of elements $x_\pi, u_\pi$ and $y_\pi, v_\pi$ are each in the same part of the partition and that $\pi$ is yet-to-linearize a \Unite{} operation with argument $(x_\pi, y_\pi)$.
\end{itemize}

\import{invariants}{union-find-tracker}

Our intricate proof that $\I$ is indeed an inductive invariant of the system and proofs of the straightforward deductions that $\I$'s invariance implies the invariance of $\I_L$ and $\I_S$, thereby proving the strong linearizability of the union find implementation can be found at: 

{\scriptsize
\url{https://github.com/visveswara/machine-certified-linearizability/blob/master/UnionFindTracker.tla}
}


==> implementations/queue-old.tex <==
\begin{figure}[H]\fbox{\begin{minipage}\textwidth		
\begin{algorithmic}[1]
    \Statex
    \Statex {\bf Base Objects:}
    \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
        \item $X$ is a F\&Inc/read register initialized to 1.
        \item $Q[1, 2, \ldots]$ is an infinite FAS/read/write array, where each $Q[i]$ is initialized to $\bot$.
    \end{itemize}
\end{algorithmic}

\begin{algorithmic}[1]
    \Statex 
    \State \cmdprocedure $\O.\Enqueue_{\pi}(v_{\pi})$
    \State \tab $i_{\pi} \gets \FAInc{X}$
    \State \tab $Q[i_{\pi}] \gets v_{\pi}$
    \State \tab \cmdreturn $\ack$
    \Statex
    \State \cmdprocedure $\O.\Dequeue_{\pi}()$
    \State \tab $l_{\pi} \gets X$
    \State \tab \cmdif $l_{\pi} = 1$ \cmdthen \cmdgoto $6$ 
    \Statex \tab \cmdelse $j_{\pi} \gets 1$
    \State \tab $x_{\pi} \gets \FAS{Q[j_{\pi}], \bot}$
    \Statex \tab \cmdif $x_{\pi} = \bot$
    \Statex \tab[2] \cmdif $j_{\pi} = l_{\pi} - 1$ \cmdthen \cmdgoto $6$
    \Statex \tab[2] \cmdelse
    \Statex \tab[3] $j_{\pi} \gets j_{\pi} + 1$
    \Statex \tab[3] \cmdgoto $8$
    \State \tab \cmdreturn $x_{\pi}$
\end{algorithmic}
    \caption{
        Herlihy and Wing's queue implementation.
    }
\label{impl:queue}
\end{minipage}}\end{figure}


==> implementations/queue-tracker-old.tex <==
\begin{figure}[H]\fbox{\begin{minipage}\textwidth		
\begin{algorithmic}[1]
    \Statex
    \Statex {\bf Base Objects:}
    \begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
        \item $X$ is a F\&Inc/read register initialized to 1.
        \item $Q[1, 2, \ldots]$ is an infinite FAS/read/write array, where each $Q[i]$ is initialized to $\bot$.
        \item $\M$ initialized to $\{(\sigma_0, f_0) \}$ is a meta-configuration, where $\sigma_0$ is the empty sequence, and $f_0$ maps each process $\pi \in \Pi$ to $(\bot,\bot,\bot)$.
\end{itemize}
    
\end{algorithmic}

\begin{algorithmic}[1]
    \Statex 
    \State \cmdprocedure $\Oaug.\Enqueue_{\pi}(v_{\pi})$
    \Statex \tab $\M \gets \{C' \mid \exists C \in \M : C' = invoke(C, \pi, \Enqueue_{\pi}(v_{\pi}))\}$
    \State \tab $i_{\pi} \gets \FAInc{X}$
    \Statex \tab $\M \gets \{C' \mid \exists C \in M, S \subseteq pending(C), \alpha \in Perm(S): C' = \delta^*(C, \alpha)$ 
    \Statex \tab[16] \ \ \ $\wedge \ \forall \pi' \in S : pc_{\pi'} \in \{3, 4\} \vee \pi' = \pi\}$
    % \Statex \tab $\M \gets \{C' \ | \ \exists C \in \M : C' \}$
    \State \tab $Q[i_{\pi}] \gets v_{\pi}$
    \State \tab \cmdreturn $\ack$
    \Statex \tab $\M \gets \{C' \mid \exists C \in \M : C' = return(C, \pi, $ \cmdreturn $\ack)\}$
    \Statex
    \State \cmdprocedure $\Oaug.\Dequeue_{\pi}()$
    \Statex \tab $\M \gets \{C' \mid \exists C \in \M : C' = invoke(C, \pi, \Dequeue_{\pi}())\}$
    \State \tab $l_{\pi} \gets X$
    \State \tab \cmdif $l_{\pi} = 1$ \cmdthen \cmdgoto $6$ 
    \Statex \tab \cmdelse $j_{\pi} \gets 1$
    \State \tab $x_{\pi} \gets \FAS{Q[j_{\pi}], \bot}$
    \Statex \tab \cmdif $x_{\pi} = \bot$
    \Statex \tab[2] \cmdif $j_{\pi} = l_{\pi} - 1$ \cmdthen \cmdgoto $6$
    \Statex \tab[2] \cmdelse
    \Statex \tab[3] $j_{\pi} \gets j_{\pi} + 1$
    \Statex \tab[3] \cmdgoto $8$
    \Statex \tab \cmdelse 
    \Statex \tab[2] $\M \gets \{C' \mid \exists C \in \M : C' = \delta^*(C, \pi)\}$
    \State \tab \cmdreturn $x_{\pi}$
    \Statex \tab $\M \gets \{C' \mid \exists C \in \M : C' = return(C, \pi, $ \cmdreturn $x_{\pi})\}$
    % \Statex
\end{algorithmic}
    \caption{
        Tracker $\Oaug$ for the queue implementation $\O$ presented in Figure~\ref{impl:queue}
    }
\label{impl:queue-tracker}
\end{minipage}}\end{figure}


==> implementations/rw-tracker.tex <==
\begin{figure}[h]\fbox{\begin{minipage}\textwidth		
			\begin{algorithmic}[1]
				\Statex
				\Statex {\bf Base Objects:} 
				\begin{itemize}
					\item 
					$X$ is an LL/SC register, initialized to state $(X.val, X.pset) = (\sigma_0, \nullset)$.
					\item
					$P = \{(\sigma_0, f)\}$ where $f(\pi) \mapsto (\bot, \bot,\bot)$ for all $\pi \in \Pi$.
				\end{itemize} 
			\end{algorithmic}
			
			\begin{algorithmic}[1]	
				\State \cmdprocedure $\O.read_\pi()$ 
				\Statex $P \gets \{(\sigma, g) \mid \exists (\sigma, f) \in P: f(\pi) = (\bot, \bot, \bot) \wedge g(\pi) = (read, \bot, \bot) \wedge \forall \rho \ne \pi, g(\rho) = f(\rho)\}$

				\State \tab $r_\pi \gets X.LL_\pi()$
				\Statex \tab $P \gets \{(\sigma, g) \mid \exists (\sigma, f) \in P: f(\pi) = (read, \bot, \bot) \wedge g(\pi) = (read, \bot, r) \wedge \forall \rho \ne \pi, g(\rho) = f(\rho)\}$
				
				\State \tab \cmdreturn $r_\pi$
				\Statex \tab $P \gets \{(\sigma, g) \mid \exists (\sigma, f) \in P: f(\pi) = (read, \bot, r) \wedge g(\pi) = (\bot, \bot, \bot) \wedge \forall \rho \ne \pi, g(\rho) = f(\rho)\}$
				
				\Statex
				
				\State \cmdprocedure $\O.write_\pi(v_\pi)$
				\Statex $P \gets \{(\sigma, g) \mid \exists (\sigma, f) \in P: f(\pi) = (\bot, \bot, \bot) \wedge g(\pi) = (write, v, \bot) \wedge \forall \rho \ne \pi, g(\rho) = f(\rho)\}$

				\State \tab $X.LL_\pi()$
				\Statex \tab $P \gets P$
			
				\State \tab $X.SC_\pi(v_\pi)$
				\Statex \tab 
				$
				  	P \gets \left\{ (\psi, g)\ \middle\vert	\begin{array}{l}
					\exists (\sigma, f) \in P: \\
					\tab g(\pi) = (write, v_\pi, \ack) \:\wedge \\
					\tab \forall \rho \in \Pi: (pc_\rho \ne 6 \implies g(\rho) = f(\rho)) \:\wedge \\
					\tab (\pi \in X.pset \implies (\psi = v_\pi \wedge \forall \rho \in \Pi: pc_{\rho} = 6 \implies g(\rho) = (write, v_\rho, ack) )) \:\wedge \\
					\tab (\pi \not\in X.pset \implies (\psi = \sigma \wedge \forall \rho \in \Pi: (pc_{\rho} = 6 \wedge \rho \ne \pi) \implies g(\rho) = f(\rho)))
				\end{array}\right\}
				$


				\State \tab \cmdreturn $\ack$				
				\Statex \tab $P \gets \{(\sigma, g) \mid \exists (\sigma, f) \in P: f(\pi) = (write, v, \ack) \wedge g(\pi) = (\bot, \bot, \bot) \wedge \forall \rho \ne \pi, g(\rho) = f(\rho)\}$

			\end{algorithmic}
			
			\caption{: 
				Implementation of a read/write register initialized to $\sigma_0$ from an LL/SC object $X$ initialized to $(\sigma_0, \nullset)$.
			}
			\label{impl:rw}
\end{minipage}}\end{figure}


==> implementations/rw.tex <==
\begin{figure}[h]\fbox{\begin{minipage}\textwidth		
			\begin{algorithmic}[1]
				\Statex
				\Statex {\bf Base Object:}  $X$ is an LL/SC register, initialized to state $(X.val, X.pset) = (\sigma_0, \nullset)$.
			\end{algorithmic}
			
			\begin{algorithmic}[1]	
				\State \cmdprocedure $\O.read_\pi()$ 
				\State \tab $r_\pi \gets X.LL_\pi()$
				\State \tab \cmdreturn $r_\pi$
				
				\Statex
				
				\State \cmdprocedure $\O.write_\pi(v_\pi)$
				\State \tab $X.LL_\pi()$
				\State \tab $X.SC_\pi(v_\pi)$
				\State \tab \cmdreturn $\ack$				
			\end{algorithmic}
			
			\caption{: 
				Implementation of a read/write register initialized to $\sigma_0$ from an LL/SC register $X$ initialized to $(\sigma_0, \nullset)$.
			}
			\label{impl:rw}
\end{minipage}}\end{figure}


==> implementations/union-find-tracker.tex <==
\begin{figure}[H]\fbox{\begin{minipage}\textwidth		
			\begin{algorithmic}[1]
				\Statex
				\Statex {\bf Base Objects:}  
				\begin{itemize}
				    \item
    				$x.par$ is a Read/CAS register initialized to $x.par = x$, for each node $x \in [n]$.
                    \item
                    $\M$ initialized to $\{(\sigma_0, f_0) \}$ is a meta-configuration, where $\sigma_0$ maps each $x \in [n]$ to $\{x\}$ and $f_0$ maps each $\pi \in \Pi$ to $(\bot,\bot,\bot)$.
				\end{itemize}
			\end{algorithmic}
			
			\begin{algorithmic}[1]	
				\State \cmdprocedure $\Oaug.\Find_\pi(x_\pi)$
				\Statex \tab $u_\pi \gets x_\pi$ 
                \Statex \tab 
                $\M \gets \left\{ C' \ \middle\vert	
    	                \exists C \in \M:
    					    C' = invoke(C, \pi, \Find_\pi(x_\pi))
  			    \right\}$
				% \Statex \tab $u_\pi \gets x_\pi$ 
    %             \Statex \tab 
    %             $\M \gets \left\{ (\sigma, f')\ \middle\vert	
    % 	                \exists (\sigma, f) \in \M:
    % 					    f'(\pi) = (\Find{}, x_\pi, \bot) \: \wedge
				% 			\forall \ol{\pi} \in \Pi - \{\pi\}: f'(\ol{\pi}) = f(\pi)
  		% 	    \right\}$
                
				\State  \tab \cmdwhile $u_\pi \ne u_\pi.par$ \cmddo $u_\pi \gets u_\pi.par$
				\Statex \tab \cmdif $u_\pi = u_\pi.par$ \cmdthen 
                $\M \gets \left\{ C' \middle\vert	
  	            \begin{array}{l}
    	                \exists C \in \M:
    	                    C' = \delta^*(C, \pi)
  				\end{array}
  			    \right\}$
				% \Statex \tab \cmdif $u_\pi = u_\pi.par$ \cmdthen 
    %             \Statex \tab[2] 
    %             $\M \gets \left\{ (\sigma, f')\ \middle\vert	
  	 %           \begin{array}{l}
    % 	                \exists (\sigma, f) \in \M:
    % 	                    f(\pi).res = \bot \: \wedge
    % 					    f'(\pi) = (f(\pi).op, f(\pi).arg, \max\sigma(f(\pi).arg)) \\
				% 			\tab \wedge\: \forall \ol{\pi} \in \Pi - \{\pi\}: f'(\ol{\pi}) = f(\pi)
  		% 		\end{array}
  		% 	    \right\}$
				
				\State  \tab \cmdreturn $u_\pi$
                \Statex \tab 
                $\M \gets \left\{ C'\ \middle\vert	
    	                \exists C \in \M:
    	                    C' = return(C, \pi, \cmdreturn\: u_\pi)
  			    \right\}$
    %             \Statex \tab 
    %             $\M \gets \left\{ (\sigma, f')\ \middle\vert	
    % 	                \exists (\sigma, f) \in \M:
    % 					    f'(\pi).res = u_\pi \: \wedge 
    % 					    f'(\pi) = (\bot, \bot, \bot) \: \wedge 
				% 			\forall \ol{\pi} \in \Pi - \{\pi\}: f'(\ol{\pi}) = f(\pi)
  		% 	    \right\}$

                \Statex

                \State  \cmdprocedure $\Oaug.\Unite_\pi(x_\pi, y_\pi)$ 
				\Statex \tab $u_\pi \gets x_\pi$; $v_\pi \gets y_\pi$
                \Statex \tab 
                $\M \gets \left\{ C'\ \middle\vert	
    	                \exists C \in \M:
    					    C' = invoke(C, \pi, \Unite_\pi(x_\pi, y_\pi))
  			    \right\}$
    %             \Statex \tab 
    %             $\M \gets \left\{ (\sigma, f')\ \middle\vert	
    % 	                \exists (\sigma, f) \in \M:
    % 					    f'(\pi) = (\Unite{}, (x_\pi, y_\pi), \bot) \: \wedge
				% 			\forall \ol{\pi} \in \Pi - \{\pi\}: f'(\ol{\pi}) = f(\pi)
  		% 	    \right\}$

				\Statex \tab \cmdwhile $\true$ \cmddo
				
				\State  \tab[2] \cmdif $u_\pi = v_\pi$ \cmdthen \cmdgoto~line~8
				\Statex \tab[2] \cmdelif $u_\pi < v_\pi$ \cmdthen \cmdif $\CAS{u_\pi.par, u_\pi, v_\pi}$ \cmdthen \cmdgoto~line~8
				\Statex \tab[2] \cmdelif $u_\pi > v_\pi$ \cmdthen \cmdif $\CAS{v_\pi.par, v_\pi, u_\pi}$ \cmdthen \cmdgoto~line~8
				
				\Statex \tab[2] \cmdif $(u_\pi = v_\pi) \vee (u_\pi < v_\pi \wedge u_\pi = u_\pi.par) \vee (u_\pi > v_\pi \wedge v_\pi = v_\pi.par)$ \cmdthen 
			    \Statex \tab[3]   	
                $\M \gets \left\{ C'\ \middle\vert	
    	                \exists C \in \M:
    					    C' = \delta^*(C, \pi)
  			    \right\}$
				% \Statex \tab[2] \cmdif $u_\pi = v_\pi$ \cmdthen 
			 %   \Statex \tab[3]   	
    %             $\M \gets \left\{ (\sigma, f')\ \middle\vert	
    % 	                \exists (\sigma, f) \in \M:
    % 					    f'(\pi) = (f(\pi).op, f(\pi).arg, \ack) \: \wedge
				% 			\forall \ol{\pi} \in \Pi - \{\pi\}: f'(\ol{\pi}) = f(\pi)
  		% 	    \right\}$
				% \Statex \tab[2] \cmdelif $(u_\pi < v_\pi \wedge u_\pi = u_\pi.par) \vee (u_\pi > v_\pi \wedge v_\pi = v_\pi.par)$ \cmdthen 
				% \Statex \tab[3]
    %             $\M \gets \left\{ (\sigma', f')\ \middle\vert	
  	 %           \begin{array}{l}
    % 	                \exists (\sigma, f) \in \M:
    % 	                    f(\pi).res = \bot \\
    % 					    \tab \wedge\: f'(\pi).res = (f(\pi).op, f(\pi).arg, \ack) \\
    % 					    \tab \wedge\: \forall \ol{\pi} \in \Pi - \{\pi\}: f'(\pi) = f(\pi) \\ 
				% 			\tab \wedge\: \forall z \in \sigma(f(\pi).arg.x) \cup \sigma(f(\pi).arg.y): \\
				% 			\tab[2] \sigma'(z) = \sigma(f(\pi).arg.x) \cup \sigma(f(\pi).arg.y) \\
				% 			\tab \wedge\: \forall z \not\in \sigma(f(\pi).arg.x) \cup \sigma(f(\pi).arg.y): \\
				% 			\tab[2] \sigma'(z) = \sigma(z) \\
  		% 		\end{array}
  		% 	    \right\}$


				\State  \tab[2] \cmdwhile $u_\pi \ne u_\pi.par$ \cmddo $u_\pi \gets u_\pi.par$
				
				\State  \tab[2] \cmdwhile $v_\pi \ne v_\pi.par$ \cmddo $v_\pi \gets v_\pi.par$
				
				\State  \tab \cmdreturn \ack
                \Statex \tab 
                $\M \gets \left\{ C'\ \middle\vert	
    	                C' = return(C, \pi, \cmdreturn\: \ack)
  			    \right\}$
    %             \Statex \tab 
    %             $\M \gets \left\{ (\sigma, f')\ \middle\vert	
    % 	                \exists (\sigma, f) \in \M:
    % 					    f'(\pi).res = \ack \: \wedge 
    % 					    f'(\pi) = (\bot, \bot, \bot) \: \wedge 
				% 			\forall \ol{\pi} \in \Pi - \{\pi\}: f'(\ol{\pi}) = f(\pi)
  		% 	    \right\}$
				
			\end{algorithmic}
			
			\caption{ 
				Tracker $\Oaug$ for the union find implementation $\O$ presented in Figure~\ref{impl:union-find}.
			}
			\label{impl:union-find-tracker}
\end{minipage}}\end{figure}


==> implementations/union-find.tex <==
\begin{figure}[H]\fbox{\begin{minipage}\textwidth		
			\begin{algorithmic}[1]
				\Statex
				\Statex {\bf Base Objects:}  
				\begin{itemize}
				\item
    		$x.par$ is a Read/CAS register initialized to $x.par = x$, for each node $x \in [n]$.
				\end{itemize}
			\end{algorithmic}
			
			\begin{algorithmic}[1]	
				\State \cmdprocedure $\O.\Find_\pi(x_\pi)$
				\Statex \tab $u_\pi \gets x_\pi$ 
				\State  \tab \cmdwhile $u_\pi \ne u_\pi.par$ \cmddo $u_\pi \gets u_\pi.par$
				\State  \tab \cmdreturn $u_\pi$

                \Statex

                \State  \cmdprocedure $\O.\Unite_\pi(x_\pi, y_\pi)$ 
				\Statex \tab $u_\pi \gets x_\pi$; $v_\pi \gets y_\pi$
				\Statex \tab \cmdwhile $\true$ \cmddo
				\State  \tab[2] \cmdif $u_\pi = v_\pi$ \cmdthen \cmdgoto~line~8
				\Statex \tab[2] \cmdelif $u_\pi < v_\pi$ \cmdthen \cmdif $\CAS{u_\pi.par, u_\pi, v_\pi}$ \cmdthen \cmdgoto~line~8
				\Statex \tab[2] \cmdelif $u_\pi > v_\pi$ \cmdthen \cmdif $\CAS{v_\pi.par, v_\pi, u_\pi}$ \cmdthen \cmdgoto~line~8
				\State  \tab[2] \cmdwhile $u_\pi \ne u_\pi.par$ \cmddo $u_\pi \gets u_\pi.par$
				\State  \tab[2] \cmdwhile $v_\pi \ne v_\pi.par$ \cmddo $v_\pi \gets v_\pi.par$
				\State  \tab \cmdreturn \ack
				
			\end{algorithmic}
			
			\caption{ 
				Jayanti and Tarjan's implementation of a union find object on $n$ nodes $\{1,2,\ldots,n\}$ each initially in its own singleton part of the partition, i.e., the initial state is $\sigma_0: [n] \to \mathcal{P}([n])$ defined by $\forall x \in [n], \sigma_0(x) = x$.
			}
			\label{impl:union-find}
\end{minipage}}\end{figure}


==> invariants/union-find-tracker.tex <==
\begin{figure}[H]\fbox{\begin{minipage}\textwidth		
\caption{
Invariant $\I$ of $\A(\Oaug)$, where $\Oaug$ is the implementation of the union find tracker in Figure~\ref{impl:union-find-tracker}.
}
\begin{align*}
\I \equiv\: &\I_L \wedge \I_S \\
            &\wedge\: \I_{par} \wedge \I_x \wedge \I_y \wedge \I_u \wedge \I_v \wedge \I_{pc} \wedge \I_\M \\
            &\wedge\: \I_a \wedge \I_b \wedge \I_c \\
            &\wedge\: \I_{1,4} \wedge \I_2 \wedge \I_3 \wedge \I_{5,6,7} \wedge \I_8
\end{align*}

In the above expression, the various conjuncts on the right hand side are defined below.

\begin{itemize}[parsep=0pt,partopsep=0pt]
    \item
    $\I_{L} \equiv \M \ne \nullset$
    \item 
    $\I_{S} \equiv |\M| = 1$

    \item
    $\I_{par} \equiv \forall z \in [n]: z.par \in [n]$
    \item
    $\I_{x} \equiv \forall \pi \in \Pi: x_\pi \in [n]$
    \item
    $\I_{y} \equiv \forall \pi \in \Pi: y_\pi \in [n]$
    \item
    $\I_{u} \equiv \forall \pi \in \Pi: u_\pi \in [n]$
    \item
    $\I_{v} \equiv \forall \pi \in \Pi: v_\pi \in [n]$
    \item
    $\I_{pc} \equiv \forall \pi \in \Pi: pc_\pi \in [8]$
    \item
    $\I_\M \equiv \M \subseteq AtomicConfigurations$
    % \item
    % \hspace{-0.1in}
    % $\begin{array}{l}
    %         \I_{\M} \equiv 
    %         \M \subseteq AtomicConfigurations \\
    %         \tab[2] \wedge\: \forall (\sigma, f) \in \M: \forall z \in [n]: z \in \sigma(z) \\
    %         \tab[2] \wedge\: \forall (\sigma, f) \in \M: \forall w, z \in [n]: w \in \sigma(z) \implies \sigma(w) = \sigma(z)                f(\pi).res = \bot \\
    % \end{array}$
    % $\I_{\M} \equiv \M \in AtomicConfigs$
    % \item
    % $\I_a \equiv \forall (\sigma, f) \in \M: \forall z \in [n]: z \in \sigma(z)$
    % \item
    % $\I_b \equiv \forall (\sigma, f) \in \M: \forall w, z \in [n]: w \in \sigma(z) \implies \sigma(w) = \sigma(z)$
    \item
    $\I_a \equiv \forall (\sigma, f) \in \M: \forall z \in [n]: z.par \in \sigma(z)$
    \item
    $\I_b \equiv \forall (\sigma, f) \in \M: \forall w, z \in [n]: (w \ne z \wedge w.par = w \wedge z.par = z) \implies \sigma(w) \ne \sigma(z)$
    \item 
    $\I_c \equiv \forall z \in [n]: z.par \ge z$
    \item
    $\I_{1,4} \equiv \forall \pi \in \Pi: \forall (\sigma, f) \in \M: pc_\pi \in \{1,4\} \implies f(\pi) = (\bot, \bot, \bot)$
    \item
    $\I_2 \equiv \forall \pi \in \Pi: \forall (\sigma, f) \in \M: pc_\pi = 2 \implies (\sigma(u_\pi) = \sigma(x_\pi) \wedge f(\pi) = (\Find{}, x_\pi, \bot))$
    \item
    $\I_3 \equiv \forall \pi \in \Pi: \forall (\sigma, f) \in \M: pc_\pi = 3 \implies f(\pi) = (\Find{}, x_\pi, u_\pi)$
    \item
    $\I_{5,6,7} \equiv \forall \pi \in \Pi: \forall (\sigma, f) \in \M: pc_\pi \in \{5,6,7\} \implies (\sigma(u_\pi) = \sigma(x_\pi) \wedge \sigma(v_\pi) = \sigma(y_\pi) \wedge f(\pi) = (\Unite{}, (x_\pi, y_\pi), \bot))$
    \item
    $\I_8 \equiv \forall \pi \in \Pi: \forall (\sigma, f) \in \M: pc_\pi = 8 \implies f(\pi) = (\Unite{}, (x_\pi, y_\pi), \ack)$
 \end{itemize}
\label{inv:union-find}


\end{minipage}}\end{figure}

% InvF1U1           == \A p \in PROCSET: \A t \in P: (pc[p] \in InvocationLines) => (t.f[p] = NIL)
% InvF2             == \A p \in PROCSET: \A t \in P: 
%                         (pc[p] = "F2") => (t.sigma[u[p]] = t.sigma[x[p]] /\ t.f[p] = NIL)
% InvF3             == \A p \in PROCSET: \A t \in P:
%                         (pc[p] = "F3") => (t.f[p] = u[p])
% InvU234           == \A p \in PROCSET: \A t \in P:
%                         (pc[p] \in {"U2", "U3", "U4"}) => (t.sigma[u[p]] = t.sigma[x[p]] /\ t.sigma[v[p]] = t.sigma[y[p]] /\ t.f[p] = NIL)
% InvU5             == \A p \in PROCSET: \A t \in P:
%                         (pc[p] = "U5") => (t.f[p] = ACK)

% Linearizable      == P # {}


==> object-types/LL-SC.tex <==
\begin{figure}[h]\fbox{\begin{minipage}\textwidth		
\begin{type}[LL/SC register]
For a LL/SC register type that stores integer values, we have:
\label{type:llsc}
\begin{itemize}[parsep=0pt,partopsep=0pt]
    \item 
    $\Sigma = \Z \times 2^\Pi$
    \item
    $OP = \{LL, SC\}$
    \item
    $ARG_{LL} = \{\bot\}, ARG_{SC} = \Z$
    \item
    $RES = \Z \cup \{\true, \false \}$
    \item
    Transition function $\delta$ is defined as follows:
    \begin{itemize}
        \item 
        $\delta((u, S), \pi, LL, \bot) = ((u, S \cup \{ \pi\}), u)$
        \item
            $\delta((u, S), \pi, SC, v) =
            \begin{cases}
              ((v, \nullset), \true), & \text{if}\ \pi \in S \\
              ((u, S), \false), & \text{otherwise}
            \end{cases}$

    \end{itemize}
\end{itemize}
\end{type}
\end{minipage}}\end{figure}


==> object-types/read-cas.tex <==
\begin{figure}[h]\fbox{\begin{minipage}\textwidth		
\begin{type}[Read/CAS register]
For a Read/CAS register type that stores integer values, we have:
\label{type:read-cas}
\begin{itemize}[parsep=0pt,partopsep=0pt]
    \item 
    $\Sigma = \Z$
    \item
    $OP = \{Read, \CAS{}\}$
    \item 
    $ARG_{Read} = \{\bot\}, ARG_{\CAS{}} = \Z \times \Z$
    \item
    $RES = \Z \cup \{\true, \false \}$
    \item
    Transition function $\delta$ is defined as follows:
    \begin{itemize}
        \item 
        $\delta(u, \pi, Read, \bot) = (u, u)$
        \item
            $\delta(u, \pi, \CAS{}, (x, y)) =
            \begin{cases}
              (y, \true), & \text{if}\ x = u \\
              (u, \false), & \text{otherwise}
            \end{cases}$
    \end{itemize}
\end{itemize}
\end{type}
\end{minipage}}\end{figure}


==> object-types/read-write.tex <==
\begin{figure}[h]\fbox{\begin{minipage}\textwidth		
\begin{type}[read/write register]
For a read/write register type that stores integer values, we have:
\label{type:read-write}
\begin{itemize}[parsep=0pt,partopsep=0pt]
    \item 
    $\Sigma = \Z$
    \item
    $OP = \{read, write\}$
    \item
    $ARG_{read} = \{\bot\}, ARG_{write} = \Z$.
    \item
    $RES = \Z \cup \{\ack \}$
    \item
    Transition function $\delta$ is defined as follows:
    \begin{itemize}
        \item 
        $\delta(u, \pi, read, \bot) = (u, u)$
        \item
        $\delta(u, \pi, write, v) = (v, \ack)$
    \end{itemize}
\end{itemize}
\end{type}
\end{minipage}}\end{figure}


==> old-file-to-be-deleted.tex <==
\subsection{Main Theorem}

The crafting of the tracking augmentation yields a powerful technique for producing {\em machine verified proofs} of linearizability.
This technique falls out from the main theorem of this section, which reduces the complex question of whether an implementation $\O$ is linearizable to the verification of a simple invariant.
In particular, $\O$ is linearizable {\em if and only if} $\Mfull \ne \nullset$ is an invariant of $\A(\Ofull)$.

Exploiting the {\em if} direction of this theorem, we can obtain machine verified proofs of linearizability by proving the invariant in a software system such as TLAPS (Temporal Logic of Actions Proof System) or Coq.
The {\em only if} direction of the theorem assures us that this proof technique is complete.

\begin{restatable}{theorem}{maintheorem} \label{maintheorem}
	Let $\O$ be an implementation of an object of type $\tau$ initialized to state $\sigma_0$ for a set of processes $\Pi$,
	$\O$ is linearizable {\em if and only if} $\Mfull \ne \nullset$ is an invariant of $\A(\Ofull)$.
	
	(Recall that $\Ofull$ is the full tracker of $\O$ with meta-configuration $\Mfull$, and $\A(\Ofull)$ is the algorithm from Figure~\ref{alg:generator} in which processes repeatedly make calls to procedures of $\Ofull$.)
\end{restatable}

\noindent
The remainder of the section develops the necessary machinery and proves Theorem~\ref{maintheorem}.

%R^ -> P -> Configs(p)

Let $\O$ be an implementation of an object of type $\tau$ initialized to $\sigma_0$ for a set of processes $\Pi$, and
let $O$ be an atomic object with the same type and initialization, and for the same set of processes.
Finally, recall that $\Ofull$ is the full tracker of $\O$ with meta-configuration variable $\Mfull$. 

For a generic variable $V$ of any given implementation $I$, and a run $R_I$ of the generator $A(I)$, we let $V(R_I)$ denote the value of $V$ in the final configuration of $A(I)$.
We will be particularly interested in the meta-configurations $\Mfull(\Rfull)$ for runs $\Rfull$ of $\A(\Ofull)$.

By Observation~\ref{obs:augmentation}, $\O$ is linearizable if and only if the finite behaviors of $\Ofull$ are behaviors of $O$.
Our strategy to prove the main theorem thereby, will be to show that for any run $\Rfull$ of $\Ofull$, the set of atomic runs sharing its behavior will have exactly the final configurations $\Mfull(\Rfull)$.

To effectively express the above statement, we develop a bit more notation.
For any behavior $B$, we let $AtomicRuns(B)$ be the set of atomic runs that exhibit behavior $B$.
Further, for any set of atomic run $R$, we let $\C(R)$ denote the final configuration of $R$, and for a set of runs $\Rcal$, we let $\C(\Rcal) = \{\C(R) \mid R \in \Rcal \}$ denote the set of final configurations of all those runs.
For a given run $\Rfull$ of the implementation, we define $Linearizations(\Rfull) \triangleq AtomicRuns(behavior(\Rfull))$.

We are now ready to prove the key lemma that will propel the proof of Theorem~\ref{maintheorem}.

\begin{lemma}
\label{lem:mainlemma}
	Let $\Rfull$ be any finite run of $\Ofull$, then the following equality holds:
	\begin{equation*}
		\Mfull(\Rfull) = \C(Linearizations(\Rfull))
	\end{equation*}	
\end{lemma}

% We will prove Lemma~\ref{lem:mainlemma} by induction.
% For convenience, we prove the base case and induction step as separate lemmas.

\begin{proof}
		The proof is by induction on the number of events in the run $\Rfull$.
		\begin{itemize}
			\item 
			{\bf Base Case:} 
			Every implementation run $\Rfull$ with zero events is simply an initial configuration $\Cfull_0$ of algorithm $\A(\Ofull)$.
			In this case, $behavior(\Rfull)$ is the empty behavior, and thus only the empty atomic run is in $Linearizations(\Rfull) = AtomicRuns(behavior(\Rfull))$.
			The final (and only) configuration of this run is the unique initial atomic configuration $C_0 = (\sigma_0, f_0)$;
			thus $\C(Linearizations(\Rfull)) = \{(\sigma_0, f_0) \}$ which is the definition of $\Mfull(\Cfull_0)$.
			
			\item
			{\bf Induction Step:}
			Let $\Rfull_k = \Cfull_0, \ldots, \Cfull_{k-1},(\pi_k, \ell_k),\Cfull_k$ be run with $k \ge 1$ events.
			We consider the prefix-run $\Rfull_{k-1} = \Cfull_0,\ldots,\Cfull_{k-1}$, and note that the induction hypothesis states that:
			\[\Mfull(\Rfull_{k-1}) = \C(Linearizations(\Rfull_{k-1}))\]
			
			For notational convenience, we define $B_k = behavior(\Rfull_k)$ and $B_{k-1} = behavior(\Rfull_{k-1})$.
			The last line executed in $\Rfull$, i.e. $\ell_k$, can be one of three types of lines: invocation, intermediate, or return. 
			\begin{itemize}
				\item 
				\underline{Case: $\ell_k$ is an invocation $op_{\pi}(arg)$}.
				First, we show that RHS $\subseteq$ LHS.
				That is, let $L_k \in Linearizations(\Rfull_k)$; we must first prove that $\C(L_k) \in \Mfull(\Rfull_k)$. 
				To this effect, define $L_{k-1}$ to be the longest prefix of $L_k$, such that $behavior(L_{k-1}) = B_{k-1}$.
				By definition of atomic runs, $L_k$ results when $L_{k-1}$ is followed immediately by the invocation $op_{\pi}(arg)$ and subsequently by a (possibly empty) sequence of linearization steps by processes $\alpha = \alpha_1,\ldots,\alpha_h$ that are yet to linearize in $invoke(\C(L_{k-1}), \pi, op_\pi(arg))$.
				In particular, no other invocation or return events are possible, since $behavior(L_k) = B_k$ which has just the single invocation more than $B_{k-1}$.
				Thus, by definition $\C(L_k)$ results from $\pi$ invoking $op_\pi(arg)$ and $\alpha_1,\ldots,\alpha_h$ linearizing after configuration $\C(L_{k-1})$.
				Since $\C(L_{k-1}) \in \Mfull(\Rfull_{k-1})$ by the inductive hypothesis, $\C(L_k) \in EvolveInv(\Mfull(\Rfull_{k-1}), \pi, op_\pi(arg)) = \Mfull(\Rfull_k)$.
				
                Second we prove that LHS $\subseteq$ RHS.
                That is, let $C_k \in \Mfull(\Rfull_k)$, we must prove that there is a linearization $L_k$ of $\Rfull_k$ with final configuration $\C(L_k) = C_k$.
                To this effect, we note that $\Mfull(\Rfull_k) = EvolveInv(\Mfull(\Rfull_{k-1}), \pi, op_\pi(arg))$.
                That is, there is a configuration $C_{k-1} \in \Mfull(\Rfull_{k-1})$ such that $C_k$ results from $\pi$ invoking $op_\pi(arg)$ and some sequence of processes $\alpha = \alpha_1,\ldots,\alpha_h$ linearizing after $C_{k-1}$.
                By the inductive hypothesis, there is a linearization $L_{k-1}$ of $\Rfull_{k-1}$ whose final configuration is $\C(L_{k-1}) = C_{k-1}$ in which $\pi$ is idle and $\alpha_1,\ldots,\alpha_h$ are yet-to-linearize in $invoke(C_{k-1}, \pi, op_\pi(arg))$.
                Thus, the atomic run $L_k$ that extends $L_{k-1}$ with $\pi$ invoking and $\alpha$ linearizing after $C_{k-1}$ is a linearization of $\Rfull_k$ whose final configuration is $\C(L_k) = C_k$, which concludes the proof of the case.
                
				\item
				\underline{Case: $\ell_k$ is an intermediate line}.
                Since $behavior(\Rfull_k) = behavior(\Rfull_{k-1})$,
                we invoke the inductive hypothesis to get the equality:
                \[\Mfull(\Rfull_{k-1}) = \C(Linearizations(\Rfull_{k-1})) = \C(Linearizations(\Rfull_k)) \]
                Now, we observe that when $\Mfull(\Rfull_{k-1})$ is already the full set of final configurations of linearizations with the behavior $B_{k-1} = B_{k}$, evolving does not change the set, that is:
                \[\Mfull(\Rfull_k) = Evolve(\Mfull(\Rfull_{k-1})) = Evolve(\C(Linearizations(\Rfull_k))) = \C(Linearizations(\Rfull_k))\]
                Thus, we conclude the proof of the case.
                                
				\item
				\underline{Case: $\ell_k$ is a return $\text{\bf return } res$}.
				This case is very similar to the first case.
				Once again, we first show that RHS $\subseteq$ LHS.
				That is, let $L_k \in Linearizations(\Rfull_k)$; we must first prove that $\C(L_k) \in \Mfull(\Rfull_k)$. 
				To this effect, define $L_{k-1}$ to be the longest prefix of $L_k$, such that $behavior(L_{k-1}) = B_{k-1}$.
				By definition of atomic runs, $L_k$ results when $L_{k-1}$ is followed immediately by the return of $res$ and subsequently by a (possibly empty) sequence of linearization steps by processes $\alpha = \alpha_1,\ldots,\alpha_h$ that are yet to linearize in $return(\C(L_{k-1}), \pi, \cmdreturn\: res)$.
				In particular, no other invocation or return events are possible, since $behavior(L_k) = B_k$ which has just the single return more than $B_{k-1}$.
				Thus, by definition $\C(L_k)$ results from $\pi$ returning $res$ and $\alpha_1,\ldots,\alpha_h$ linearizing after configuration $\C(L_{k-1})$.
				Since $\C(L_{k-1}) \in \Mfull(\Rfull_{k-1})$ by the inductive hypothesis, $\C(L_k) \in EvolveRet(\Mfull(\Rfull_{k-1}), \pi, \cmdreturn\: res) = \Mfull(\Rfull)$.
				
                Second we prove that LHS $\subseteq$ RHS.
                That is, let $C_k \in \Mfull(\Rfull_k)$, we must prove that there is a linearization $L_k$ of $\Rfull_k$ with final configuration $\C(L_k) = C_k$.
                To this effect, we note that $\Mfull(\Rfull_k) = EvolveRet(\Mfull(\Rfull_{k-1}), \pi, \cmdreturn\: res)$.
                That is, there is a configuration $C_{k-1} \in \Mfull(\Rfull_{k-1})$ such that $C_k$ results from $\pi$ returning $res$ and some sequence of processes $\alpha = \alpha_1,\ldots,\alpha_h$ linearizing after $C_{k-1}$.
                By the inductive hypothesis, there is a linearization $L_{k-1}$ of $\Rfull_{k-1}$ whose final configuration is $\C(L_{k-1}) = C_{k-1}$ in which $\pi$ has linearized with return value $res$ and $\alpha_1,\ldots,\alpha_h$ are yet-to-linearize in $return(C_{k-1}, \pi, \cmdreturn\: res)$.
                Thus, the atomic run $L_k$ that extends $L_{k-1}$ with $\pi$ returning and $\alpha$ linearizing after $C_{k-1}$ is a linearization of $\Rfull_k$ whose final configuration is $\C(L_k) = C_k$, which concludes the proof of the case.
			\end{itemize}			 
		\end{itemize}	
\end{proof}

We are now ready to prove the main theorem.

\maintheorem*

\begin{proof}
	We will prove the theorem by showing the forward and reverse directions separately:
	\begin{itemize}
		\item 
		For the forward direction:
		assume $\Mfull \ne \nullset$ is an invariant of $\A(\Ofull)$.
		Thus, for any finite run $\Rfull$ of $\A(\Ofull)$, we note $\Mfull(\Rfull)$ is non-empty.
		So, by Lemma~\ref{lem:mainlemma}, there is a linearization $L$ of $\Rfull$.
		Since, an arbitrary finite run $\Rfull$  of $\A(\Ofull)$ is linearizable, we conclude that $\Ofull$ is linearizable.
		Since $\Ofull$ has the same behaviors as $\O$, thus $\O$ is linearizable.
		
		\item
		For the reverse direction:
		assume that $\O$ is linearizable.
		This implies $\Ofull$ is linearizable.
		So, every finite run $\Rfull$ of $\A(\Ofull)$ has at least one linearization $L$.
		Thus, by Lemma~\ref{lem:mainlemma}, $\Mfull(\Rfull)$ is non-empty.
		Since, $\Mfull(\Rfull)$ is non-empty for an arbitrary finite run $\Rfull$ of $\A(\Ofull)$, we conclude that $\Mfull \ne \nullset$ is an invariant of $\A(\Ofull)$.
	\end{itemize}
\end{proof}

\subsection{(Partial) Trackers}

The proof of Theorem~\ref{maintheorem} demonstrates that, for an implementation $\O$, the full tracker $\Ofull$ tracks ``all possible linearizations'' in its meta-configuration.
To show that $\O$ is linearizable however, it suffices to show the existence of a single linearization for every run.
That is, we need not track {\em all} linearizations, but just ensure that we track {\em at least one}.
In practice, tracking a subset of linearizations can be easier for a prover, especially one who knows the structure of the implementation well.
Thus, in general, we will be interested in a (partial) tracker, whose meta-configuration $\M$ maintains a subset of the full meta-configuration $\Mfull$.
We define such trackers.

\begin{definition}[trackers]
	Let $\O$ be an implementation of a type $\tau$ in the initial state $\sigma_0$ for a set of processes $\Pi$.
	We say $\Opart$ is a partial tracking augmentation of $\O$, if the following conditions are met:
	\begin{itemize}
		\item
		The augmenting variable set $\Omega_{aug}$ of $\Opart$ contains a meta-configuration variable $\Mpart$  that holds a set of atomic configurations.
		($\Omega_{aug}$ may also contain other additional variables.)
		
		\item
		$\Mpart$ is initialized to $\{(\sigma_0, f_0)\}$, where $f_0(\pi) = (\bot, \bot, \bot)$ for every $\pi \in \Pi$.
		
		\item
		For each type of line $\ell$ (whether invocation, intermediate, or return) in the original algorithm, the augmented line $\ellpart$ updates the tracker to ensure the new value of $\Mpart$ is a subset of the configurations that would arise by evolving $\Mpart$ according to the rules of the full tracker.
		That is, if the update of the tracker at line $\ellpart$ is $M \gets Evolve_\ell(\M)$, then:
		\begin{itemize}
		 	\item
                    	\underline{Case: $\ell$ is the invocation of $op_{\pi}(arg)$}.
                    	\begin{equation}
                      	Evolve_\ell(\Mpart) \subseteq EvolveInv(\Mpart, \pi, op_\pi(arg))
                    	\end{equation} 
                    
                    	\item
                    	\underline{Case: $\ell$ is an intermediate line of $op_{\pi}(arg)$}.
                    	\begin{equation}
                    	Evolve_\ell(\Mpart) \subseteq Evolve(\Mpart)
                    	\end{equation} 

                    	\item
                    	\underline{Case: $\ell$ is a $\cmdreturn \: res$ statement from a procedure $op_{\pi}(arg)$}.
                    	\begin{equation}
                    	Evolve_\ell(\Mpart) \subseteq EvolveRet(\Mpart, \pi, \cmdreturn\: res)
                    	\end{equation} 
		 \end{itemize}	
	\end{itemize} 
\end{definition} 

\begin{theorem}
\label{thm:partial-tracker}
	Let $\O$ be an implementation of an object of type $\tau$ initialized to state $\sigma_0$ for a set of processes $\Pi$,
	and $\Opart$ be any partial tracking augmentation of $\O$ with meta-configuration variable $\Mpart$.
	If $\Mpart \ne \nullset$ is an invariant of $\A(\Opart)$, then $\O$ is linearizable.
\end{theorem}

\begin{proof}
	Let $\Mfull$ be the meta-configuration of the full tracker $\Ofull$.
	Consider any run $\Rfull = \Cfull_0, (\pi_1, \ellfull_1), \Cfull_1, (\pi_2, \ellfull_2), \ldots$ of $\A(\Ofull)$.
	We say the run $\Rpart = \Cpart_0, (\pi_1, \ellpart_1), \Cpart_1, (\pi_2, \ellpart_2), \ldots$ of $\A(\Opart)$ is coupled with $\Rfull$, if $\Cpart_0$ has the same initialization for the private registers and objects in $\tau.\Omega$, and for each $i$, $\ellpart_i$ is the line in $\Opart$ that corresponds to $\ellfull_i$ in $\Ofull$ (i.e. these are augmentations of corresponding lines in $\O$).
	Since $\Ofull$ and $\Opart$ augment the same implementation, all runs of $\A(\Ofull)$ and $\A(\Opart)$ are coupled as $(\Rfull, \Rpart)$ in this way.  
	For coupled run $\Rfull$ and $\Rpart$, by definition of a partial tracking augmentation, it is clear that $\Mpart \subseteq \Mfull$ throughout the coupled run.
	Thus, $\Mpart \ne \nullset$ being an invariant of $\Opart$ implies $\Mfull \ne \nullset$ is an invariant of $\Ofull$.
	So, by Theorem~\ref{maintheorem}, the proof is complete.
\end{proof}

